Understanding Training Efficiency of Deep Learning Recommendation Models at Scale

The use of GPUs has proliferated for machine learning workflows and is now considered mainstream for many deep learning models. Meanwhile, when training state-of-the-art personal recommendation models, which consume the highest number of compute cycles at our large-scale datacenters, the use of GPUs came with various challenges due to having both compute-intensive and memory-intensive components. GPU performance and efficiency of these recommendation models are largely affected by model architecture configurations such as dense and sparse features, MLP dimensions. Furthermore, these models often contain large embedding tables that do not fit into limited GPU memory. The goal of this paper is to explain the intricacies of using GPUs for training recommendation models, factors affecting hardware efficiency at scale, and learnings from a new scale-up GPU server design, Zion.

==> introduction.tex <==
Deep learning recommendation algorithms have recently gained significant 
adoption to power a wide variety of products. For example, Google
utilizes 
deep candidate generation and ranking models to produce video suggestions 
to users in Youtube~\cite{Covington:RecSys2016},
and
designs deep learning 
recommendation models to personalize mobile app suggestions for 
Google Play~\cite{Cheng:dlrs2016}.
Microsoft leverages deep learning recommendation models for news 
suggestions~\cite{Elkahky:www2015}, Netflix for personalized 
entertainment~\cite{raimond:2018}, Alibaba for product 
recommendation~\cite{zhou:arxiv2018}. 
At Facebook, personalization and ranking use cases are powered 
by deep learning recommendation models: Instagram stories are 
ranked with multi-stage deep neural networks (DNNs)~\cite{Medvedev:2019}, 
Newsfeed Ranking and Search tasks are also built upon 
DNNs~\cite{hazelwood:hpca2018,Song:arxiv2020}. 
Depending on the specific use cases, features and model architectures
exhibit diverse characteristics -- leading to a variety of deep 
recommendation models in Facebook's production training environment. 

The rise of deep learning recommendation models is rapid.
Over the  last 18-month period,
we have witnessed the compute capacity for 
recommendation model training has quadrupled at Facebook datacenter 
fleets~\cite{naumov:arxiv2020}. Among the total AI training cycles 
at Facebook, more than 50\% has been devoted to training deep learning 
recommendation models. Thus, understanding and improving the training 
efficiency for the wide variety of deep learning recommendation models 
in the production environment is key to increasing the overall AI 
infrastructure efficiency. 

\begin{figure}[th]
\centering
\includegraphics[width=0.9\columnwidth]{figures/intro_marked.pdf}
\caption{Throughput of three production models with different hardware and embedding table (EMB) placement strategies.}
\label{speedup_quality_example}
\end{figure}

% Summarize in the second paragraph [cjw]
% Training recommendation models account for around 50\% of all AI training cycles in our heterogeneous large-scale data-center at Facebook. Further, the demand for more compute resources has been growing rapidly. Therefore, understanding and improving the efficiency of recommendation models is key to increasing the overall efficiency of our datacenters.

% Summarize in the first paragraph [cjw]
% There are variety of personalization use cases at Facebook. NewsFeed Ranking, Ads Ranking, Stories Ranking, Instagram Explore, Marketplace Ranking are some of the examples. Further, each of the use case has diverse features and characteristics that are unique to themselves. 

% Introduce the primary elements of deep learning recommendation 
% models (DLRMs) -- MLPs and embedding tablees
Despite having similar overall structure and components, personal recommendation models can have diverse characteristics based on model architecture and input configurations. This can cause large variations in utilization of the servers across different training runs.
Moreover, depending on the model configuration the most efficient hardware choice (i.e. CPU only vs GPU) could be different for each configuration. These configurations include: dense and sparse features, feature interaction, MLP (multi-layer perceptron) stack etc. 
Figure~\ref{speedup_quality_example} shows that, depending on the model
architecture and configuration, training throughput can vary
for three different production models across different Facebook 
training systems. 
% This following sentence can be the introduction of the training steps 
% for Section 3
% Figure~\ref{training_configs} shows overview of the steps in training a general recommendation model and it highlights the components that are commonly configured differently across different training runs of a model type.

As described by Hazelwood et al.~\cite{hazelwood:hpca2018}, while language and 
vision models are trained on the eight-GPU BigBasin production 
systems, the majority of deep learning recommendation model training runs on 
clusters of dual-socket CPU production machines. This is because of the large 
memory capacity and bandwidth requirement of embedding tables in
our deep learning recommendation models.
The memory capacity of embedding 
tables have increased drastically from tens of GBs to TBs in the industry~\cite{zhao2020distributed},
while the memory bandwidth consumption also increases quickly with the increasing number of embedding table lookup operations up to hundreds~\cite{zhou2019deep}.

The goal of this paper is threefold.
First, we present workload
characteristics of training recommendation models at scale.
Second, we characterize the effect of 
model configurations, such as dense and sparse features, batch size, 
embedding table hash size, MLP dimensions, on training throughput. 
Third, we enable GPU-training of three
production-scale deep learning recommendation models using 
Facebook's customized eight-GPU server Big Basin and scale-out GPU 
server Zion.
We quantify factors affecting 
hardware efficiency by comparing training throughput and model 
qualities on these GPU and CPU architectures.

Prior studies proposed methodologies to parameterize deep learning models and study the characteristics~\cite{wang2020systematic} however training personal recommendation models are not studied
in a systematic way in the literature. Other existing studies analyze the architectural implications of inference of recommendation models~\cite{gupta2020deeprecsys, gupta2020architectural}, however training is different than inference in two significant ways. First, training configurations highly effect model quality, which is not a concern during inference. Second, training is commonly done in a distributed way to be able process the high volume of down-sampled input data quickly and distributed training requires a gradient synchronization step that is not needed during inference.


Given the diverse characteristics of different model configurations, the most efficient hardware choice for each training workflow run might be different. In a heterogenous data-center with a mix of CPU and GPU servers, deciding which server is optimal to use for a given model configuration may not easily be determined by ML engineers who train their model. There are existing methods to predict the performance of code on a different hardware, such as predicting GPU performance using CPU code~\cite{ardalani2015cross}, using a roofline model~\cite{williams2009roofline}, or using a binary predictor
approach~\cite{baldini2014predicting}. However such methods may not be applicable to recommendation models since 
large memory capacity requirement of embedding tables requires different software infrastructure for handling the placement of the
embedding tables given the limited memory of GPUs.

In this work, we shed light on how different model configurations of recommendation models effect training efficiency at scale.
Key contributions of this paper are \textcolor{blue}{[Summarize the key results (with concrete numbers) and insights gained over this paper, for example, from the various result sections.]}:
\begin{itemize}
    \item We explain in detail how the model configurations affect hardware utilization and efficiency at scale. We analyze both model architecture and system configurations (Section~\ref{model_configs},~\ref{hardware}).
    \item We identify general characteristics that make workloads more or less amenable to GPU acceleration (Section~\ref{efficiency}).
    \item We show case studies of three different production models and compare their power efficiency, performance and model accuracy on CPU and GPU platforms (Section~\ref{case_studies}).
\end{itemize}



